Deploying and Evaluating LLMs to Program Service Mobile Robots

Recent advancements in large language models (LLMs) have spurred interest in using them for generating robot programs from natural language, with promising initial results. We investigate the use of LLMs to generate programs for service mobile robots leveraging mobility, perception, and human interaction skills, and where accurate sequencing and ordering of actions is crucial for success. We contribute CodeBotler, an open-source robot-agnostic tool to program service mobile robots from natural language, and RoboEval, a benchmark for evaluating LLMs' capabilities of generating programs to complete service robot tasks. CodeBotler performs program generation via few-shot prompting of LLMs with an embedded domain-specific language (eDSL) in Python, and leverages skill abstractions to deploy generated programs on any general-purpose mobile robot. RoboEval evaluates the correctness of generated programs by checking execution traces starting with multiple initial states, and checking whether the traces satisfy temporal logic properties that encode correctness for each task. RoboEval also includes multiple prompts per task to test for the robustness of program generation. We evaluate several popular state-of-the-art LLMs with the RoboEval benchmark, and perform a thorough analysis of the modes of failures, resulting in a taxonomy that highlights common pitfalls of LLMs at generating robot programs. We release our code and benchmark at https://amrl.cs.utexas.edu/codebotler/.

==> 05-results-old.tex <==
\section{Benchmark Results And Analysis}

\begin{comment}
We hope to gain insights into the capabilities of different SOTA LLMs for generating service robot programs, so we perform analysis using the RoboEval benchmark. We are particularly interested in two questions:
1. first, how do different LLMs perform in generating service robot tasks in the RoboEval benchmark?
2. then, when a generated service robot LMP fails, what is the cause of the failures?
To explore these two questions, we [talk about setup]. In the following subsection, we discuss each question in order.

Q1:
[Each LLM's overall performance in generating code] Explain CDF
Takeaway: there is still a fraction of prompts that result in no successful completions

[Task level performance ]
Explain Bar Chart
Takeaway: this needs to be worked on

[Prompt level performance]
Explain Error Bar
Takeaway: changes in the phrasing of the prompt can result in substantial performance variations even for the same intended task

[Common sense reasoning]
Explain Common Sense Reasoning Bar Chart
-- We have noticed that LLMs tend not to be able to successfully generate programs for the tasks with common sense reasoning, so we are interested in understanding whether needing to perform common sense reasoning is the cause of the LLMs underperforming. [talk about how we create the plot]. 
Takeaway: Although LLMs are not always proficient at common sense reasoning, they nevertheless demonstrate some ability to do so. This indicates that the causes of LLMs underperforming are attributed to a variety of reasons we discuss next. 

Q2:
Given that LLMs are not perfect, we want to understand the cause of failures for LLMs to generate robot programs. To facilitate this analysis, we group all failures into three categories [explain categories]. 

 Takeaway: Code-writing LLMs are better at making fewer Pythonn errors even though they in general perform worse at generating robot programs, which probably is due to the size of the model or the extensive training/tuning on the proprietary models. 

In the following subsection, we will discuss each in detail.
   
[Python Error Analysis]
Takeaway:
    1. GPT3.5 and GPT-4 suffer from Name Error where the variables being used are not defined.  
    2. TypeError stands out for PaLM and CodeLLama --- they generate programs that use the types incorrectly (e.g. adding string to int)
    3. Starcoder encounters timeout error where programs that require for/while loop

[Robot Execution Error Analysis]
Takeaway:
    1. LLMs suffer from hallucination problems
    2. Service robot programs need to be aware of the robot's internal state (pick and place). The occurrences of this kind of error indicate that LLMs might suffer from complex tasks that require the LLMs to keep track of the robot's internal state when generating programs.

[Task Completion Error Analysis]
Takeaway:
    1. There is a large percentage of the errors that are a result of the task "come back and tell me".  [describe this command a little more]. [add the explanation of this phenomenon. ]


New Section: Improving performance
From the above analysis section, we observe that a significant portion of the errors happen in the simulator. Hence, we can catch these errors before deployment. To do so, we can use rejection sampling. 

Takeaway:
- We observe it can improve performance to certain degrees. Yet, this approach alone is not enough because
1. There is still a significant number of times an LLM might generate a program that pass in simulator but still fails in the evaluator
2. No matter how many times we regenerate, we cannot get a correct program for certain prompts -- some prompts will always cause an LLM to fail to generate a program. 

Hence, rejection sampling is only effective to a certain degree and a more sophisticated approach still needs to be developed. 


\end{comment}

\begin{figure}[h]
    \centering
    \resizebox{\columnwidth}{!}{
        \input{figures/cdf.pgf}
    }
    \caption{Cumulative Distribution Function (CDF) curves of each LLM's pass@1 score over all prompts. A perfect LLM would have a horizontal line crossing the y-axis at $100\%$ -- this LLM can generate for $100\%$ of the prompts with a pass@1 score of 1.}
    \label{fig:performance-cdf}
\end{figure}





\begin{figure*}[h]
    \centering
    \resizebox{\textwidth}{!}{
        \input{figures/error_h.pgf}
    }
    \caption{Causes of failures for LMPs on the \roboeval{} benchmark.}
    \label{fig:cause-of-failures}
\end{figure*}
In this section, we present the results and insights of evaluating the correctness of LLM-generated robot programs using the \roboeval{} benchmark.
We evaluate five LLMs using \codebotler{} and \roboeval{}:
\begin{enumerate*}
    \item GPT-4 \cite{openai2023gpt4}, 
    \item GPT-3.5 \cite{brown2020language} (\texttt{text-davinci-003}), and 
    \item PaLM2 \cite{anil2023palm} (\texttt{text-bison-001}) as state-of-the-art API-only proprietary models; and 
    \item CodeLlama \cite{rozière2023code} (\texttt{Python-34b-hf}) and 
    \item StarCoder \cite{li2023starcoder} as open-access models.
\end{enumerate*}
% To begin with, we choose a blend of the state-of-the-art proprietary (GPT-4, GPT-3.5/text-davinci-003, PaLM2/text-bison-001) and open-source (CodeLlama/Python-34b-hf, StarCoder) language models, and generate programs for every task in the \roboeval{} benchmark. 
For all generations, we set the temperature to $T = 0.2$, and nucleus sampling with top $p = 0.95$. We empirically evaluate the following questions:

\begin{enumerate}
    \item What is the performance of different LLMs on the RoboEval benchmark? Additionally, how does the performance vary with:
    \begin{enumerate*}
        \item different tasks;
        \item the need for open-world knowledge; and
        \item variations in objects of interest for the same task?
    \end{enumerate*}
    \item What are the causes of failure for LMPs on the RoboEval benchmark?
    \item How can code generation for robot tasks be improved?
\end{enumerate}


\subsection{Performance Of LLMs On The RoboEval Benchmark}
We generate 50 robot program completions for every prompt in the \roboeval{} benchmark using each of the LLMs. We check the programs evaluated using the \roboeval{} tests to compute the pass@1 metric~\cite{humaneval} of each LLM for each prompt. 
\figref{performance-cdf} shows the Cumulative Distribution Function (CDF) of each LLM's pass@1 score over all prompts. 
%In terms of pass@1 score, optimal performance begins at a value of 1 and reduces to 0 as the performance degrades. 
At any point $x,y$ on the CDF curve, $y\%$ of all prompts achieve a pass@1 score of $\geq x$ -- the ``perfect'' performance would thus be the $y=100\%$ line, implying that all ($100\%$) prompts have a pass@1 score of $1.0$. 
% The closer a CDF curve to the $y=100\%$ line, the better the distribution of the LLM's performance is over the dataset.
For visual clarity, we truncate the x-axis at 0.02 since all CDF plots eventually hit 100\% (since $100\%$ of the programs for any LLM has a pass@1 score of $\geq 0$).

% \jb{You should not draw undue attention to GPT-4. We aren't advertising for OpenAI. Just state which model performs the best, and then state that even the best performing model...}


\figref{performance-cdf} shows that the top-performing model (GPT-4) can generate programs for 67.5\% of the prompts with a pass@1 score of 1. 
As the pass@1 score is relaxed, for every LLM, an increasing number of the prompts result in completions that meet or exceed the pass@1 score. However, there is still a fraction of prompts that result in no successful completions -- which varies by LLM ($48.75\%$ for StarCoder, to $1.25\%$ for GPT-4).
% While LLMs can produce a higher percentage of prompts when the pass@1 score criteria are relaxed, all of the models are unable to generate all the prompts with any positive pass@1 score. 
% This suggests that current LLMs, even the most advanced ones, may sometimes struggle to consistently generate successful robot programs from natural language prompts.\jb{This is too negative a conclusion. Can we soften it a bit?}
 
 % struggle to generate a correct program for certain prompts.\jb{How is this evident from the CDF?} This suggests that the current LLMs still face challenges if used for production-ready deployment. \jb{What is ``production-ready deployment''? Just talk about what is the focus of this paper --- }
 
 % One interesting observation from \figref{performance-of-LLMs}(a) is that despite the size of CodeLlama (34B) being significantly smaller than proprietary models, its performance is catching up with the PaLM2 model.
 % \jb{What does ``is catching up with'' mean? Also how do you know that it is significantly smaller than PaLM2? There is not public data of its size. Remove this statement.}
 % Further finetuning the open-access models with domain-specific data might close the gap. \jb{This is conjecture. Do not include conjecture, just factual results and inferences that can be drawn from evidence.}
 
 In the following subsections, we investigate how different aspects of a task can affect LLMs' performance in generating robot programs.

\subsubsection{Task Performance Breakdown}
We compute the average pass@1 score of the 5 prompt paraphrases for each task and present them in a bar chart. \subfigref{performance-bar}{a} displays each LLMs' performance breakdown across all \roboeval{} benchmark tasks. 
We observe significant variations across the tasks --- most LLMs can reliably generate programs for the \texttt{SayGoodDay} task, while every LLM but GPT-4 fails for all prompts in the \texttt{LunchTime} task.
Furthermore, within each task, there are often significant variations across LLMs --- for example, in the \texttt{HalloweenShopping} task, mean pass@1 scores range from $0.98$ (GPT-4) to $0.12$ (PaLM2) to $0$ (StarCoder). 

\subsubsection{The Effect Of Prompt Variations}
\subfigref{performance-bar}{a} also includes an error bar for each LLM and task that spans from the best pass@1 score to the worst pass@1 score within 5 prompts of each task in the \roboeval{} benchmark. We note a considerable disparity between the best and worst pass@1 scores within the same task. This suggests that changes in the phrasing of the prompt can result in substantial performance variations even for the same intended task.

% On the right, we show a table of detailed scores of each LLM on each of the task prompts. From the tasks, it can be observed that Mail Delivery is the most challenging task with all LLMs but GPT-4 fails on this task. This task involves almost all aspects of the eDSL. The models seem to confuse about "asking people to put the main in the basket" with "picking up the mail themselves."   

\subsubsection{Open World Knowledge Analysis}
To evaluate the capability of LLMs in handling open-world knowledge during program creation, we modify the \roboeval{} evaluator to only check for the open-world knowledge constraints. For example, in the \texttt{GrilledCheese} task, the \roboeval{} evaluator checks for whether the program provides the \texttt{bread} and \texttt{cheese} options. 
\subfigref{performance-bar}{b} shows the performance of each LLM on the four open-world knowledge tasks. 
All LLMs, including StarCoder which is primarily trained on open-source code, demonstrate some ability to handle tasks associated with open-world knowledge. Yet, this ability is limited and can be inconsistent. Moreover, the difference between the performance when checking only for open-world knowledge and performing the complete task (\eg{} \texttt{LunchTime} in \subfigref{performance-bar}{a} \vs{} \subfigref{performance-bar}) is attributed to a variety of modes of failure, which we analyze next.

% In general, LLMs perform ok at solving open-world knowledge tasks. Even StarCoder, a solely trained on code open-source model, is able to reason about open world knowledge in some cases. Moreover, we observe that there is a significant performance difference for these 4 tasks between \figref{performance-of-LLMs}(b) and \figref{performance-of-LLMs}(c), indicating that LLMs suffer more from other reasons.

% The emergent capabilities of LLMs include open-world knowledge which is beneficial to carry out daily tasks. We analyze each language model's capabilities in understanding open-world knowledge by designing 4 specific tasks among those 16 tasks. We evaluate only the common-sense reasoning part of the benchmark, such as "choose beef jerky over donut when being asked for a savory option." As shown in \figref{openworld}, we observe that starcoder, an open-source LLM only trained on Github codes, also contains some open world knowledge.

\begin{figure*}[h]

    \subfloat[The LLMs' performance with respect to different max resampling limits. \\All LLMs improve in performance as the max resampling limit increases. ]{%
        \resizebox{.62\textwidth}{!}{\input{figures/resample_cdf.pgf}
        }
        \label{subfig:cdf-after-resampling}%
    }
    \hspace{-1cm}
    \subfloat[CDF curves of percentage of LMPs that can be successfully executed over different maximum resampling Limits]{%
        \resizebox{.4\textwidth}{!}{\input{figures/resample_till_no_crash.pgf}
        }
        \label{subfig:cdf-of-resampling-count}%
    }
    \caption{Performance improvement using rejection sampling approach.}
\end{figure*}

% To evaluate the robustness of LLMs, we compare the different prompt paraphrases within each task. in Table, we show the best and the worst pass@1 score along with the average pass@1 score. For tasks that do not completely fail, we observe that oftentimes there is a huge difference between the passs@1 for different paraphrases ranging from all succeesful of pass@1 to all failing. This matches the current view that prompt can affect LLM performance significantly (cite here). 


% \jb{List of figures:
% \begin{enumerate}
%     \item Overall CDF for all LLMs on RoboEval
%     \item Table of pass@k for each task, and overall, by LLM. rows: {heading, task1, ... taskN, Overall} columns:{heading, GPT4, GPT3.5, ...} 
%     \item [Appendix] Same as above, but per prompt. Group the prompts by task.
%     \item Distribution vs. task and prompt - number overlay
%     \item [Appendix] Table of number of unique traces and programs vs. task and prompt
% \end{enumerate}
% }




% \begin{figure*}[h]
%     \begin{center}
%     \resizebox{\textwidth}{!}{
%         \input{figures/heatmap.pgf}
%     }
%     \end{center}
%     \caption{Heatmap of pass@1 for All LLMs}
% \end{figure*}

\subsection{Causes of Failures of LMPs on the \roboeval{} Benchmark}
% \jb{List of figures:
% \begin{enumerate}
%     \item Table of Execution errors
%     \item Table of Evaluation errors
% \end{enumerate}
% }

For LLM-generated programs that fail in the \roboeval{} benchmark, we analyze the different modes of failure. We classify these failures into three categories: 
\begin{enumerate*}
    \item \texttt{Python Errors}, including syntax errors, runtime errors, and timeout errors;
    \item \texttt{Robot Execution Errors}, that occurs when a program attempts to execute an infeasible action, such as navigating to a non-existent (hallucinated) location; and
    \texttt{Task Completion Errors}, where the program runs correctly in the simulator but does not complete the intended task.
\end{enumerate*}
We use \roboeval{}'s symbolic simulator to detect and classify \texttt{Python Errors} and  \texttt{Robot Execution Errors}, and we use \roboeval{}'s evaluator to capture the \texttt{Task Completion Errors}. 

\subfigref{cause-of-failures}{a} shows a breakdown of these failure categories for each LLM. Python errors are particularly pronounced for GPT-3.5 and PaLM2, but are rare for models specialized for code completion (CodeLlama and StarCoder).
The distribution of errors between \texttt{Robot Execution Errors} and \texttt{Task Completions Errors} varies between LLMs ($4.1\%$ vs. $18.0\%$ for GPT-3.5, $23.1\%$ vs. $23.2\%$ for PaLM2, $31.0\%$ vs. $20.4\%$ for CodeLlama, $29.5\%$ vs. $35.7\%$ for StarCoder).
% In addition, the GPT series predominantly suffers from the task completion error; the CodeLlama suffers mostly from the robot execution error; and, PaLM2 and StarCoder suffer equally from the robot execution error and the task completion error. 
\subfigref{cause-of-failures}{b} shows the specific error breakdown of Python Error types \cite{python-doc} for each LLM.
In the following subsections, we further analyze the types of robot execution errors and task completion errors.

% \subsubsection{Native Python Error}
 % \figref{cause-of-failures}b shows the specific error breakdown of the \texttt{Native Python Error}. While there are numerous built-in Python errors, a few of them are responsible for the majority of errors. The GPT series frequently encounters name errors due to the presence of undefined variables in the generated code. Palm2 and Codellama mainly face type errors, often trying to add strings. On the other hand, StarCoder primarily deals with timeout errors, suggesting difficulties with "while loops" that may lead to endless iterations.
 

\subsubsection{Robot Execution Error}
To investigate the causes of failures of LLM-generated programs in the \roboeval{} symbolic simulator, we analyzed the traces of all failing programs, and found that there are 6 root causes  of robot execution errors: 
 \begin{enumerate*}
     \item GoToInvalidLocation: the program calls \texttt{go\_to} with an invalid (hallucinated) location;
     \item PlaceNoObject: the program attempts to place an object without holding one;
     \item PickWhileHolding: the program calls \texttt{pick} to attempt to pick up an object while already holding another;
     \item AskNoPerson: the program calls \texttt{ask} at a location with no person nearby;
     \item PickInvalidObject: the program calls \texttt{pick} with a non-existent (hallucinated) object; and 
     \item AskInvalidOptions: the program calls \texttt{ask} with an empty list of options for the interacting person to choose from.
 \end{enumerate*}   
\subfigref{cause-of-failures}{c} shows the distribution of types of robot execution errors for each LLM. We find that GoToInvalidLocation accounts for a significant fraction of errors for PaLM2, CodeLlama, and StarCoder, while the remainder of errors vary across the LLMs.
Hallucination appears to be a significant cause of errors (GoToInvalidLocation and PickInvalidObject) for most LLMs ($33.7\%$ for GPT-3.5, $67.7\%$ for PaLM2, $73.2\%$ for CodeLlama, and $80.5\%$ for StarCoder).
 
 % From our observations, GPT-4 primarily encounters the AskInvalidOptions error. GPT-3.5 tends to misplace the \texttt{ask} command. The other three LLMs frequently face the GoToInvalidLocation error, suggesting these models might mistakenly invent locations based on task instructions. Furthermore, these LLMs also struggle with the PickWhileHolding and PickInvalidObject errors, indicating potential challenges in relating their instructions to the real world.

\subsubsection{Task Completion Error}
Even when an LLM-generated program executes without any runtime errors, it may fail to complete the intended task. To understand the causes of such task failures, we classify every temporal check in the \roboeval{} benchmark into one of the following categories:
 \begin{enumerate*}
     \item SayAtLocation/AskAtLocation/ManipulationAtLocation/CheckEntityAtLocation: The task requires executing a specific action (\texttt{say}, \texttt{ask}, \texttt{pick}, \texttt{place} or \texttt{check}) at a specific location, but the program fails to do so;
     \item Initial/Terminal: The program does not accurately perform an initial or final action;
     \item EventOrdering: The program does not carry out actions in the prescribed sequence;
     \item Location: The program commands the robot to visit a location irrelevant to the task; and, 
     \item ExhaustiveSearch: The program does not visit all locations required to successfully complete the task.
 \end{enumerate*}
\subfigref{cause-of-failures}{d} shows the distribution of types of task completion errors for each LLM. We notice that the most common task completion errors in each LLM are the SayAtLocation error and the Initial/Terminal error. These two types of errors constitute the majority of task completion errors, making up $100\%$ of the errors in GPT-4, $95.7\%$ in GPT-3.5, $66.9\%$ in PaLM2, $79.9\%$ in CodeLlama, and $76.0\%$ in StarCoder.

After analyzing the programs that produce these errors, we find that most of these errors are related to a recurring statement in different tasks: \emph{``Come back and tell me..."}. This statement is often used in tasks in which we want a service robot to go to a different location, complete a task, and then return to us with an update on its progress. However, some programs fail for these tasks because the LLMs do not use the \texttt{get\_current\_location} primitive to record the robot's starting location, and as a result, the robot fails to return to its starting point.
 
% In \figref{cause-of-failures}d, we can see the distribution of task completion errors, which reveals that all LLMs fail for similar reasons. The most common error is the \textbf{SayAtLocation}, followed by the \textbf{Initial/Terminal} error. Upon analyzing the programs that produce these errors, we found that most of the mistakes are related to the "Come back and tell me" statement in a task. This statement is often used in tasks where we want to command a service robot to perform a task and then update us on its progress.
 
 
 % This requires the LLMs to remember the robot's initial position before initiating the tasks and then revert to that position afterward. However, the LLMs seem to struggle with this.
 

% It is interesting that all LLMs suffer from the say at location and correct start/terminal states. By taking a deeper look, it appears a recurring problem the program suffers from is that the robot fails to return to its starting location, which is a desirable capability we want the robot to have: "Go do something and come back and report to me."  (should we investigate why this is the case?)

% Aside from failing to return to the original location, we observe that GPT series are almost error-free. The trailing error for PaLM and CodeLlama are event ordering and exhaustive search (give reason why this is the case).


\subsection{Improving Code Generation For Robot Programs}
% \jb{List of figures:
% \begin{enumerate}
%     \item CDFs of improvement - including 0,4,8,infity max samples
%     \item CDF of how many samples until no execution errors
% \end{enumerate}
% }
After analyzing the different modes of the LMP\cite{codeaspolicies2022} failures, we investigate how to improve the success rate of the LMPs. Since the \texttt{Python Errors} and the \texttt{Robot Execution Errors} occur in the symbolic simulator, we can detect most of these errors prior to deploying the program on a robot. This allows us to perform rejection sampling --- we can keep prompting an LLM for a new program until the program executes successfully in the symbolic simulator or we reach the preset maximum retry limit. 

To apply this strategy to any arbitrary task, we only assume the robot has prior knowledge about its environment's map. However, we do not make any assumptions about the robot's knowledge regarding the presence of objects or humans in the environment or how a human might respond to the robot's questions. As a result, rather than using the predetermined world states in the symbolic simulator to evaluate the correctness of any particular task in the \roboeval{} benchmarks, we modify the symbolic simulator to produce random outputs for the \texttt{ask} and \texttt{is\_in\_room} primitive functions. To ensure consistent behavior of an LMP across different world states, we execute it multiple times inside a stochastic symbolic simulator. We deem the LMP successful only if it performs correctly in all executions. If the LMP fails, we invoke the LLM to generate another program.

Figure~\ref{subfig:cdf-after-resampling} demonstrates how each LLM's performance in robot program generation varies with increasing maximum retry thresholds. As the retry limit is raised, the performance of LLMs improves. Figure~\ref{subfig:cdf-of-resampling-count} shows a CDF plot of each LLM's maximum retry limits over all prompts. It is noteworthy that the majority of LLMs are unable to generate an executable program even after 10 regeneration attempts. This observation indicates that these LLMs will likely fail to produce a functional program for certain input prompts.


% (redo)
% However, even though \figref{cause-of-failures}a indicates that successful completions generally outnumber task completion errors, the distribution of these erroneous programs isn't consistent. This results in only modest enhancements in overall performance. Figure~\ref{subfig:cdf-of-resampling-count} reveals that, with the exception of GPT-4, all the other LLMs will still face errors within the symbolic simulator, irrespective of the number of program resampling attempts.





% Observing \figref{native-python-error}, there is a significant number of errors caught by the symbolic simulator. We devise a simple technique that upon receiving an error, we would ...






